Commuting Local Hamiltonians Beyond 2D

Commuting local Hamiltonians provide a testing ground for studying many of the most interesting open questions in quantum information theory, including the quantum PCP conjecture and the existence of area laws. Although they are a simplified model of quantum computation, the status of the commuting local Hamiltonian problem remains largely unknown. A number of works have shown that increasingly expressive families of commuting local Hamiltonians admit completely classical verifiers. Despite intense work, the largest class of commuting local Hamiltonians we can place in NP are those on a square lattice, where each lattice site is a qutrit. Even worse, many of the techniques used to analyze these problems rely heavily on the geometry of the square lattice and the properties of the numbers 2 and 3 as local dimensions. In this work, we present a new technique to analyze the complexity of various families of commuting local Hamiltonians: guided reductions. Intuitively, these are a generalization of typical reduction where the prover provides a guide so that the verifier can construct a simpler Hamiltonian. The core of our reduction is a new rounding technique based on a combination of Jordan's Lemma and the Structure Lemma. Our rounding technique is much more flexible than previous work, and allows us to show that a larger family of commuting local Hamiltonians is in NP, albiet with the restriction that all terms are rank-1. Specifically, we prove the following two results: 1. Commuting local Hamiltonians in 2D that are rank-1 are contained in NP, independent of the qudit dimension. Note that this family of commuting local Hamiltonians has no restriction on the local dimension or the locality. 2. We prove that rank-1, 3D commuting Hamiltonians with qudits on edges are in NP. To our knowledge this is the first time a family of 3D commuting local Hamiltonians has been contained in NP.

==> qutrits.tex <==
\section{Qutrit commuting Hamiltonians beyond the 2D lattice}
\label{sec:qutrit_beyond_2d}
In \cite{Irani_IJ2023_CommutingLocalHamiltonian}, the authors show that by restricting the geometry from general
two-dimensional polygonal complexes to a two-dimensional \emph{square lattice}, they can move beyond qubits (as
considered in both \cite{Schuch_Sch2011_ComplexityCommutingHamiltonians, Irani_IJ2023_CommutingLocalHamiltonian}) to
qutrits. In this section, we show that this restriction to the 2D lattice is unnecessary, and in fact
$(k,3)$-\twodclh{} is contained in $\cNP$.
\qutritclhnp*
The key idea is to apply the same semi-separable reduction from
\cite{Irani_IJ2023_CommutingLocalHamiltonian}, but rather than applying the 1D argument of
\cite{Schuch_Sch2011_ComplexityCommutingHamiltonians} (which highly depends on the geometry of the square lattice), we
apply a generalization of triangulation argument of \cite{Aharonov_AKV2018_ComplexityTwoDimensional}. At a high level, we
\begin{enumerate}
    \item Construct a triangulation of the 2D complex such that each triangle $T \in \mc T$ has a ``center'' term $H_c$
        where each of $H_T$'s neighbors are fully contained in $T$.
    \item For some qutrit register $\reg R$ in the support of $H_T$, we show that we can apply the semi-separable
        reduction, which poses restrictions on the local algebra on terms touching $\reg R$ (see \Cref{lem:restrictions}).
    \item Given these restrictions, there is a projector $\pi_{\reg R}$ (provided by the prover), such that in
        $\pi_{\reg R} H \pi_{\reg R}$, some term originally adjacent to $\reg R$ can be treated as acting trivially on
        $\reg R$, or $\reg R$ is reduced to a classical register.
    \item This allows us to put a corner of the co-triangulation through the punctured hole, which ensures that all
        terms are $2$-local after grouping registers according to the co-triangulation.
\end{enumerate}

The first item above is direct from \cite{Aharonov_AKV2018_ComplexityTwoDimensional}. The remainder of this section is
dedicated to giving the details for the last three steps.

\subsection{Item 2: Removing semi-separable qutrits}
\label{sec:remove_semi_separable}
We first state two key lemmas proved in \cite{Irani_IJ2023_CommutingLocalHamiltonian} which will be crucial for our
proof.

\begin{definition}[Semi-Separable Qudit]
    Let $q$ be a qudit with terms $H_1, \dots, H_k$ acting non-trivially on it. Take some non-trivial direct sum
    decomposition $\mc H_q = \oplus_i \mc H_q^{(i)}$. If all but one of the terms $H_i$ keeps all subspaces $\mc
    H^{(i)}_q$ invariant, then we say that $q$ is \emph{semi-separable}.
\end{definition}

\begin{lemma}[Semi-Separable Self Reduction \cite{Irani_IJ2023_CommutingLocalHamiltonian}]
    \label{lem:self_reduction}
    Let $H = \sum_i H_i$ be a CLH instance and $q$ be a semi-separable qudit as above, with corresponding decomposition $\mc H_q =
    \oplus_i \mc H_q^{(i)}$. Let $H_0$ be the Hamiltonian term which does not keep the decomposition invarint. We define
    the $i$-th reduced Hamiltonian $H^{(i)} = \sum_j H^{(i)}_j$ by letting $\pi_q$ be the projector onto $\mc H_q^{(i)}$
    and,
    \begin{itemize}
        \item Reducing the Hilbert space of $q$ from $\mc H_q \rightarrow \mc H_q^{(i)}$
        \item $H^{(i)}_j = \pi_q H^{(i)}_j \pi_q$ for all $i > 0$
        \item $H^{(0)}_j = \text{round}(\pi_q H^{(i)}_j \pi_q)$
    \end{itemize}
    where $\text{round}(\cdot)$ is the map which rounds all eigenvalues smaller than $1$ to $0$ (and thus outputs a
    projector). Then, the resulting Hamiltonian $H^{(i)}$ is a commuting local Hamiltonian and furthermore,
    \[
        \lambda(H) = 0 \iff \exists j \st \lambda(H^{(j)}) = 0
    \]
\end{lemma}

In \cite{Irani_IJ2023_CommutingLocalHamiltonian}, this transformation is performed over the entire Hamiltonian, which
ensures that globally there are no semi-separable qudits. When the qudit dimension is $3$,
\cite{Irani_IJ2023_CommutingLocalHamiltonian} show that this restricts the possible algebras on each qutrit $q$.

\begin{lemma}[Restrictions on Hamiltonians without Semi-Separable Qutrits]
    \label{lem:restrictions}
    Let $H$ be a qutrit CLH instance on the 2D lattice without semi-separable qutrits. Then, consider any qutrit $q$,
    and surrounding terms $P_1, P_2$ and $Q_1, Q_2$, where the $P$-type terms one interact on $q$ and same for the
    $Q$-type terms. Then the algebras $\mc A_q(P_1), \mc A_q(P_2)$ and $\mc A_q(Q_1), \mc A_q(Q_2)$ in one of the
    following ``ways,''
    \begin{itemize}
        \item $(1,1,1) \times (1,1,1)$
        \item $(1,1,1) \times (1,2)$
        \item $(1,1,1) \times (3)$
        \item $(3) \times (3)$
    \end{itemize}
    Each tuple indicates the dimension of each subspace $H_q^{(i)}$ in the decomposition induced by either the
    $P$-type terms or the $Q$-type terms.
\end{lemma}

\begin{remark}[Locally no semi-separable qutrits]
    \label{rem:locally_not_semi_separable}
    In the proof of \Cref{lem:restrictions} it turns out that we do not need $H$ to be globally free of semi-separable
    qutrits. Instead, we only need that $q$ and a \emph{specific} neighbor $q'$ (determined by the local algebras on
    $q$\footnote{Specifically, this neighbor $q'$ is determined by which of the pairs of diagonal terms $(\tilde H_1,
        \tilde H_3)$ or $(\tilde H_2, \tilde H_4)$ commute in a $(2,1)$ way, and then which term acts trivially within
    the 2-dimensional subspace}) not be semi-separable. Formally,
    \begin{enumerate}
        \item We perform the self reduction \Cref{lem:self_reduction} on $q$. $q$ is now not semi-separable.
        \item Consider the local algebras on $q$; to apply \Cref{lem:restrictions}, there is a neighboring qutrit $q'$
            which must not be semi-separable.
        \item This time apply \Cref{lem:self_reduction} on $q'$; crucially this does not affect the local algebra on
            $q$, and thus doesn't change the necessary neighbor $q'$.
        \item Finally, $q$ and $q'$ are both not semi-separable and we can apply \Cref{lem:restrictions}.
    \end{enumerate}
\end{remark}

\begin{figure}[!ht]
\centering
\begin{tikzpicture}[scale=1.5,
        classical/.style={draw,circle,inner sep=0pt,minimum size=5pt},    
        quantum/.style={fill,circle,inner sep=0pt,minimum size=5pt},
        alglabel/.style={font=\tiny}
    ]

    % label plaquettes
    \draw[fill=gray!20] (0,1) rectangle node[midway] {$\tilde H_1$} ++ (1,1) ;
    \draw[fill=gray!20] (0,0) rectangle node[midway] {$\tilde H_2$} ++ (1,1) ;
    \draw[fill=gray!20] (1,0) rectangle node[midway] {$\tilde H_3$} ++ (1,1) ;
    \draw[fill=gray!20] (1,1) rectangle node[midway] {$\tilde H_4$} ++ (1,1) ;

    \node[quantum,label={[label distance=-0.1cm]above right:$q$}] (q) at (1,1) {};
\end{tikzpicture}
\caption{The qutrit $q$ and surrounding grouped operators.}
\label{fig:local_neighborhood}
\end{figure}

On its face, \Cref{lem:self_reduction} and \Cref{lem:restrictions} only apply to degree-4 qutrits, but we've promised a
proof for the general 2D complex. In order to apply the above lemma, we'll group the terms $H_1, \dots, H_k$ acting
non-trivially on $q$ into $4$ terms, with
\[
    \tilde H_i = H_{(i-1)\cdot \floor{k/4}} + \dots H_{\min(i \cdot \floor{k/4}, k)},\ i \in [4]
\]
where the grouped terms are arranged as in \Cref{fig:local_neighborhood}.\footnote{One might wonder why this does not
allow us to reduce any 2D CLH to a 2D CLH on a square lattice. In general, this operation can blow up the local qudit
dimension, and furthermore, it is not clear that this grouping can be done in a globally consistent way.} By
\Cref{rem:locally_not_semi_separable}, this grouping needs to be applied to $q$ and a neighbor $q'$. Such a grouping is
demonstrated in \Cref{fig:second_grouping}. After this process, we are left with a qutrit $q$ on which we can apply
\Cref{lem:restrictions}.

\input{figures/second_grouping.tex}

\subsection{Item 3: Puncturing holes}
\label{sec:puncture}
In this section, we use \Cref{lem:restrictions} along with the grouping in the previous section to show that enough
holes can be puncture in the Hamiltonian. We case on whether the decomposition has a pair of terms commuting in a
$(1,1,1)$-way, or both commute in a $(3)$-way. For ease of presentation, we rename $\tilde H_1$ and $\tilde H_3$ as
$P_1$ and $P_2$, and $\tilde H_2$ and $\tilde H_4$ as $Q_1$ and $Q_2$. Thus, $P_1, P_2$ only touch on a single
qutrit, and same for $Q_1, Q_2$.

\paragraph{Case: $(1,1,1)$} Without loss of generality, say that $P_1, P_2$ commute in a $(1,1,1)$-way. The
prover provides a projection $\pi_q$, corresponding to a $1$-dimensional subspace such that,
\begin{align}
    \tr\Brac{\vphantom{\prod_{h \in S}}(\id - P_1)(\id - Q_1)\right.&\left.(\id - P_2)(\id - Q_2) \prod_{h \in S} (\id -
    h)} > 0\\
    \label{eq:111_first}
                                   &\iff \tr\Brac{\pi_q(\id - P_1)\pi_q(\id - Q_1)\pi_q (\id - P_2)\pi_q(\id - Q_2) 
                                   \prod_{h \in S} (\id - h)} > 0
\end{align}
where again $S$ is the set of terms not adjacent to $q$. Since $\pi_q$ is a rank-1 projector, write $\pi_q = \ketbra
\psi$. Furthermore, $P_1, P_2$ are consistent with $\pi_q$ and thus we can write $P_1 = \psi \otimes \tilde P_1$ and
$P_2 = \psi \otimes \tilde P_2$. This allows us to rewrite \Cref{eq:111_first} as,
\[
    (\ref{eq:111_first}) = \tr\Brac{(\psi - \psi \otimes \tilde P_1)(\psi - \psi Q_1 \psi)(\psi - \psi \otimes \tilde P_2)
    (\psi - \psi Q_2 \psi) \prod_{h \in S} (\id - h)}
\]
This object corresponds to a valid commuting local Hamiltonian, where the qutrit is restricted to the $1$-dimensional
subspace spanned by $\psi$. Clearly the $P$-type terms commute with each other and with the $Q$-type terms. Furthermore,
since $Q_1$ and $Q_2$ only interact on $q$ and they are both restricted $\ket \psi$ on $q$, these two commute as well.
Therefore, we are left with a classical qudit on $q$ and this can be factored out of the system.

\vspace{1em}
\noindent \textbf{Case: $(3) \times (3)$} This implies that within the full Hilbert space of the qutrit, one of $P_1$
and $P_2$ act trivially on $q$ (WLOG let it be $P_1$) and one of $Q_1, Q_2$ act trivially on $q$ (let it be $Q_1$).
Then, we're immediately done, as there is already a hole in the Hamiltonian at qutrit $q$.

\subsection{Item 4: Triangulation}
To conclude the proof, for each triangle $T \in \mc T$, we take the terms $H_T$ at the center, and identify one of the
qutrits $q$ on which it acts non-trivially. Following this, we perform the grouping from
\Cref{sec:remove_semi_separable} to remove semi-separable qutrits. After performing puncturing (\Cref{sec:puncture})
some term adjacent $q$ will act trivially on $q$. Crucially, the quasi-Euclidian condition of the triangulation allows
us to take the triangles $T$ large enough such that each set of grouped terms are not adjacent to each other, and fully
contained within a single triangle.

\input{figures/triangulation.tex}

We now define the co-triangulation of $\mc T$ which will define the new qudits in the final Hamiltonian. Pick the
centers $c$ of the co-triangulation to be in the "trivialized" component, and extend paths from $c$ to (the midpoint of) each edge of the
surrounding triangle, taking care that each path starting from $c$ initially crosses different edges. Since any two
terms $H, H'$ only intersect on a single edge, this ensures each term is contained in at most 2 distinct segments of the
co-triangulation. Finally, group all qudits within each triangle of the co-triangulation. Since no term acts
non-trivially at the corners of the triangulation and all remaining terms cross at most one path of the
co-triangulation, the result is a $2$-local commuting Hamiltonian.

